Realistic Modeling of Human Timings for Wearable Cognitive Assistance

Wearable Cognitive Assistance (WCA) applications present a challenge to benchmark and characterize due to their human-in-the-loop nature. Employing user testing to optimize system parameters is generally not feasible, given the scope of the problem and the number of observations needed to detect small but important effects in controlled experiments. Considering the intended mass-scale deployment of WCA applications in the future, there exists a need for tools enabling human-independent benchmarking. We present in this paper the first model for the complete end-to-end emulation of humans in WCA. We build this model through statistical analysis of data collected from previous work in this field, and demonstrate its utility by studying application task durations. Compared to first-order approximations, our model shows a ~36% larger gap between step execution times at high system impairment versus low. We further introduce a novel framework for stochastic optimization of resource consumption-responsiveness tradeoffs in WCA, and show that by combining this framework with our realistic model of human behavior, significant reductions of up to 50% in number processed frame samples and 20% in energy consumption can be achieved with respect to the state-of-the-art.

==> old_model.tex <==
\todo[inline]{Rewrite! New model!}

As expressed in \cref{ssec:plos}, for ~\cite{olguinmunoz:impact2021} we collected timing and task performance data for \num{40} participants performing a \num{169}-step task, guided by a \ac{WCA}, as well as personality trait scores for each participant.
For this paper, we use this data to construct a probabilistic model for the generation of realistic execution times.
The data is pre-processed to group execution time values by level of neuroticism, previous \acp{TTF}, and duration of impairment.
The resulting collections of execution times represent the distributions of these values for users with specific levels of neuroticism, interacting with systems at specific states of impairment and recent histories of impairment.
These distributions can then be sampled to produce new, realistic execution times.
In the following, we detail the step-by-step processing of this data and construction of the probabilistic model.

We employ a cleaned and re-parameterized copy of the aforementioned timing data.
The \num{6760} data points are arranged in a table together with identifiers for the subjects, their neuroticism score, and a sequence number for each step.

\begin{table}[]
    \centering
    \caption{%
        Default bins used for model parameter levels.
        For impairment, values were rounded to three decimal places.
    }
    \label{tab:defaultbins}
    % \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}lccc@{}}
        \toprule
        \textbf{Parameter} & \textbf{Low}     & \textbf{Medium}      & \textbf{High}         \\ \midrule
        Neuroticism        & \( [0, 0.5) \)   &                      & \( [0.5, 1.0] \)      \\
        Impairment         & \( [0, 1.482) \) & \( [1.482, 3.198) \) & \( [3.198, \infty) \) \\
        Duration           & \( [0, 5) \)     & \( [5, 10) \)        & \( [10, \infty) \)    \\ \bottomrule
    \end{tabular}%
    % }
\end{table}

We begin by discretizing normalized neuroticism into \emph{low} and \emph{high} ranges, and \ac{TTF} into three ranges by splitting the data on the 3-quantiles; we will refer to these ranges of \ac{TTF} as \emph{low}, \emph{medium}, and \emph{high impairment}.
\cref{tab:defaultbins} shows the exact values used for these ranges.

The next steps of processing are slightly more complex.
For the data of each subject (which we will refer to as a \emph{run}), we shift the execution times by one sample such that each \ac{TTF} measurement (and therefore, impairment level) is associated with the execution time for the next step.
This comes directly from our discussions in \cref{sec:background} and~\cite{olguinmunoz:impact2021}.
Users notice the impairment of the current step only when they have finished it, and thus system impairment has no effect on the execution time of the current step, but directly affects the next one.

We then assign a label to each sample indicating the class of the most recent transition in impairment level in the run.
In other words, for each recorded step, we look back until we find a step with a different level of impairment and assign a label to the current step according to whether that change was from a higher to a lower level of impairment or vice-versa.
% However, if the current step is too far from the latest transition in impairment (by default, more than \num{8} steps), it is instead marked as \emph{no transition}; this label is also used for steps at the beginning of each run which have no previous transition in impairment.
% This labeling allows us to capture the behavior described in \cref{item:remain} of \cref{ssec:plos}.

Finally, we assign a number to each sample corresponding to \emph{how long} the system has been under the current level of impairment, in number of steps.
% This count resets whenever this combination changes.
This value is subsequently discretized into three levels; \emph{short}, \emph{medium}, and \emph{long duration} (again, refer to \cref{tab:defaultbins} for the exact values used).

% The results of this processing on the samples from \cref{tab:data:exectime} can be seen in \cref{tab:data:exectime:processed}.
Three examples of the effect of this discretization and processing on the data are presented in \cref{fig:timing}.
Specifically, we showcase how
\begin{enumerate*}[itemjoin={{; }}, itemjoin*={{; and}}]
    \item higher neuroticism leads to higher mean execution times as impairment goes up (\cref{fig:timing:impneurvsetime})
    \item duration has both a speed-up and slow-down effect on execution times, depending on the level of impairment (\cref{fig:timing:durvsetime})
    \item transitions from higher to lower levels of impairment lead to higher mean execution times when compared to steps far away from a transition, or from a transition from lower to higher levels of impairment (\cref{fig:timing:imptransvsetime})
\end{enumerate*}.


Finally, we present a step-by-step breakdown of how this data is subsequently used to generate realistic execution times.
A model which uses this processed data to generate execution times needs to maintain variables for duration, previous impairment, and most recent transition.
At the beginning of each step, it:
\begin{enumerate}
    \item Checks whether any change in impairment has occurred.
          If it has, it resets duration to \num{1} and updates the transition variable accordingly.
          If not, it increases the duration variable by one.
        %   unless that increase causes it to exceed the threshold of steps required to forget a transition.
        %   If that's the case, instead the model resets duration to \num{1} and sets the transition variable to ``no transition''.
    \item Discretizes the updated duration value.
    \item Finds all samples with binned neuroticism, impairment and duration matching the state of the system.
    If, and only if, the current duration falls within the \emph{short} duration bin, this data is further bisected according to the current value of the transition variable.
    \item Randomly samples the filtered data to obtain a realistic execution time value.
          \begin{itemize}
              \item Alternatively, a distribution can be first be fitted to the filtered samples.
                    The model then samples the theoretical distribution instead of the empirical samples.
          \end{itemize}
    \item Finally, updates the stored impairment value with the new impairment and proceeds to the next step.
\end{enumerate}

We use Python~\num{3.10} to implement two variants of the above described timing model.
The first of these samples execution times directly from the empirical data from~\cite{olguinmunoz:impact2021}; we will refer to it hereafter as the \emph{empirical model}.
The second corresponds to one which first fits a theoretical \ac{exGaussian} distribution to the data before sampling; we will refer to this one as the \emph{theoretical model}.
The \ac{exGaussian} distribution was chosen due to the vast body of research supporting its suitability for the modeling of the timing of human actions~\cite{Rohrer1994analysis,Palmer2011shapes,Marmolejo2022generalised}.
Collectively, we will refer to both these models interchangeably as the \emph{realistic models} or \emph{second-order models}.
\todo[inline]{Explain why using ExGaussian?}

We also implement two simpler reference timing models:
\begin{enumerate*}[itemjoin={{; }}, itemjoin*={{; and }}]
    % \item a model which returns a constant execution time, corresponding to the mean execution time of all samples associated with the lowest impairment and the shortest duration
    \item a model which randomly samples from the raw data without any grouping
    \item a model which fits an \ac{exGaussian} distribution to the raw data, without any grouping, and then randomly samples from it  
\end{enumerate*}.
We will refer to these models individually as the \emph{naive} and \emph{fitted-naive} model, respectively, and collectively as the \emph{firt-order models}.

\begin{figure*}
    \centering
    \includegraphics[width=.9\textwidth]{figs/model_comp_controlled_ttf.png}
    \begin{tabular}{ll >{\columncolor[HTML]{EAEAEA}}r >{\columncolor[HTML]{EAEAEA}}r rr}
    \toprule
    {} & {} & \multicolumn{2}{>{\columncolor[HTML]{EAEAEA}}c}{\ac{TTF} \( = \) \SI{0}{\second}} & \multicolumn{2}{c}{\ac{TTF} \( = \) \SI{5}{\second}} \\
    {Model} & {Neuroticism} & {Total Duration} & {Diff.\ w.r.t.\ fitted-naive} & {Total Duration} & {Diff.\ w.r.t.\ fitted-naive} \\
    \midrule
    fitted-naive & & \SI{575.54}{\second} & & \SI{1082.28}{\second} & \\
    \multirow[c]{2}{*}{empirical} & low & \SI{509.39}{\second} & \SI{-11.49}{\percent} & \SI{1071.99}{\second} & \SI{-0.95}{\percent} \\
    & high & \SI{536.48}{\second} & \SI{-6.79}{\percent} & \SI{1235.65}{\second} & +\SI{14.17}{\percent} \\
    \multirow[c]{2}{*}{theoretical} & low & \SI{505.22}{\second} & \SI{-12.22}{\percent} & \SI{1073.49}{\second} & \SI{-0.81}{\percent} \\
    & high & \SI{536.31}{\second} & \SI{-6.82}{\percent} & \SI{1235.70}{\second} & +\SI{14.18}{\percent} \\
    \bottomrule
    \end{tabular}
    \caption{
        Comparison of the total duration of \num{100}-step tasks for different models in the controlled \ac{TTF} setup.
        The table shows a detailed breakdown of durations for the fitted-naive, empirical, and theoretical models at the lowest and highest \acp{TTF}, as well as relative differences with respect to the corresponding fitted-naive baseline for each case.
    }\label{fig:ctrlttf}
\end{figure*}


We first compare these models using a controlled, ideal setup with \num{25} constant, linearly distributed \acp{TTF} in the \SIrange[]{0}{5}{\second} range.
For each \ac{TTF}, the models execute \num{30} independent repetitions of a \num{100} step task.

We show the results of these runs in \cref{fig:ctrlttf}.
Two interesting behaviors of the realistic models can be noticed in this plot.
One, all realistic models are faster than the reference models at the lowest \ac{TTF}.
When compared to the fitted-naive model, the reduction in total duration was on average \textasciitilde\SI{12}{\percent} for realistic models with low neuroticism, and \textasciitilde\SI{6.8}{\percent} for the same models with high neuroticism.

Two, at the highest \ac{TTF}, \emph{only} the high neuroticism models show any significant difference in duration with respect to the reference models.
For \ac{TTF} \(=\) \SI{5.0}{s}, the high neuroticism realistic models were on average \textasciitilde\SI{14.18}{\percent} slower than the fitted-naive model, whereas the low neuroticism models showed no significant relative difference in duration.

These behaviors clearly stem from the effects identified in \textcite{olguinmunoz:impact2021}, described in \cref{ssec:plos}.
At low levels of impairments, i.e.\ small \acp{TTF}, the speed-up effect dominates, bringing execution times to a minimum and consequently resulting in shorter total durations.
On the other hand, at high levels of impairment, the slow-down (pacing) effect starts to take over, pushing step execution times and total durations up.
However, only in the high neuroticism case do execution times eventually surpass the reference model, which is in line with our findings with respect to the modulating effects of neuroticism.

\medskip

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/EdgeDroid2ExperimentalSetup.png}
    \caption{%
        Experimental setup used to study the implications of the realistic models of human behavior for \ac{WCA}.
        We deploy containerized instances of the client-server loop running the models on a testbed consisting of \num{10} Raspberry Pi clients connected to a cloudlet over a \ac{COTS} \acs{IEEE} \num{802.11}n access point.
    }\label{fig:expsetup}
\end{figure}

These models are then integrated into client software for communicating with an adapted and instrumented version of the Gabriel~\cite{Chen2015LEGO,Chen2018application} \ac{WCA} backend running variants of the LEGO task.
In the following we use these client-server loops together with the testbed show in \cref{fig:expsetup} to illustrate the implications of the realistic timing models.
Our goal is to understand the consequences of taking second order effects into consideration when modeling execution times, versus simply relying on first-order statistics.

\todo[inline]{Update with new deployment, 802.11b/g wifi.}

We deploy an increasing number of client-server loops (\numlist{1;4;7;10} loops) in parallel on the testbed and record the resulting timing metrics.
These setups are repeated \num{5} times per model for better statistical representativeness; realistic models parameterized with \emph{low} (\num{0.0}) and \emph{high} (\num{1.0}) neuroticism are considered separate models for the purpose of this experiment.
The task used for all repetitions corresponds to a variant of the \num{169}-step tasks used in~\cite{olguinmunoz:impact2021}, truncated to \num{45} steps plus a special initial trigger step. 

\medskip

\begin{figure*}
    \centering
    \begin{subfigure}[t]{\columnwidth}
        \centering
        \includegraphics[width=.8\textwidth]{figs/numclients_vs_duration.png}
        \caption{%
            Consequences of decreased system responsiveness due to resource and network congestion.
            At lower levels of resource contention, the realistic models outperform the naive one due to the speed-up effect described in \cref{sec:background}.
            However, at higher levels of contention, the behavioral slow-down of the realistic models due to higher \acp{TTF} takes over.
        }\label{fig:scaling_duration}
    \end{subfigure}%
    \hspace{\fill}%
    \begin{subfigure}[t]{\columnwidth}
        \centering
        \includegraphics[width=.8\textwidth]{figs/neuroticism_vs_duration.png}
        \caption{%
            Modulating effects of neuroticism on task duration.
            Realistic models parameterized with high neuroticism are on average \SI{7.3}{\percent} slower than the reference model, and \SI{3.37}{\percent} slower than the same models instead parameterized with low neuroticism.
        }\label{fig:neuro_duration}
    \end{subfigure}%
    \caption{Results for both scenarios described in \cref{ssec:model:verification}. Error bars indicate the \SI{95}{\percent} \ac{CI}.}
\end{figure*}

\cref{fig:scaling_duration} illustrates the results for scenario \labelcref{verification:scaling}.
It showcases the important behaviors of the realistic models which are not captured by the naive, non-adaptive model.
On one hand, the realistic models (and by extension, humans) are actually faster than the naive model by up to \SI{4.37}{\percent} in a deployment with no resource contention.
This is due to the speed-up effect described in \textcite{olguinmunoz:impact2021} --- humans get faster as a task progresses with a high system responsiveness.

On the other, the realistic models experience a mean slowdown of about \SI{5.13}{\percent} at the highest level of resource contention (\num{10} concurrent loops) when compared to the naive model, even though only about \SI{22}{\percent} of \acp{TTF} in this scenario reach the medium impairment level and practically no \acp{TTF} pass threshold for the highest level of impairment.
This showcases that the additional user slow-down due to reduced system responsiveness, originally described in \textcite{olguinmunoz:impact2021}, causes a noticeable and significant extension of system utilization time, even at lower and medium levels of impairment.

\medskip

We illustrate the results of scenario \labelcref{verification:neuro} in \cref{fig:neuro_duration}, showcasing the modulating effects of neuroticism in a medium-impairment setup.
The realistic models were on average \SI{3.8}{\percent} slower than the reference naive model when configured with a low level of neuroticism, and \SI{7.3}{\percent} slower when configured with a high neuroticism.
In this scenario, an average of \SI{50}{\percent} of all recorded \acp{TTF} fell within the medium impairment range, and about \SI{26.6}{\percent} within the high impairment range, showing that the effects of behavioral slow-down are considerable even in moderately impaired systems. 

\medskip

The results for scenarios \labelcref{verification:scaling,verification:neuro} showcase the importance and potential impact of realistic models for the study of \ac{WCA} applications.

\todo[inline]{Finish this subsection.}

==> outline.tex <==
\section{Outline of paper}

Main research question:

\emph{Implications of the interdependence between human behavior and system responsiveness in WCA applications}

\begin{enumerate}
    \item Introduction
    \item Background and related work
        \begin{enumerate}
            \item What is WCA?
            \item Why is it interesting?
            \item Example applications and systems.
            \item Studying the impact of WCA on edge computing systems (why do we need a model for WCA?).
            \item Trade-offs: responsiveness (i.e. sampling speed) vs network load.
            \item Discuss how responsiveness relates to execution times and subsequently to system utilization.
            \item How to study these effects? Experimentally, with a model.
            \item Introduce model of WCA, refer back to PLOS paper. 
            % \item Impact of sampling schemes on system load.
            % \item Include examples from other systems (control theory).
            % \item Previous work on sampling in WCA.
            % \item Research on sampling is hampered by the lack of a model for WCA.
            % \item Previous approaches to understanding WCA behavior and modeling it.
        \end{enumerate}
    \item Model for WCA
        \begin{enumerate}
            \item Reiterate reasons for model: correlations between step execution time and system responsiveness
            \item Discuss base data from PLOS paper
                \begin{enumerate}
                    \item Timing
                    \item Frames
                \end{enumerate}
            \item Timing model
            \item Frame generation model
            \item Discuss effects of neuroticism (? for this we would need Bobby I think)
            \item Implementation in Python
        \end{enumerate}
    \item Validation of WCA Model
    \begin{enumerate}
        \item Reference model implementation (naive model)
        \item Comparison between naive, empirical, theoretical model using zero-wait sampling.
        \begin{enumerate}
            \item Scaling behavior (1, 5, and 10 clients?)
        \end{enumerate}
        \item Highlight behaviors captured by realistic models that are not present in naive model.
        \item Primarily, the spread in durations. Realistic models get faster in optimal conditions, but also react more strongly to lowered responsiveness.
    \end{enumerate}

    \item Studying implications of responsiveness-network load trade-offs using the model
    \begin{enumerate}
        \item Sampling strategies as a way to alter this trade-off.
        \item Present basic strategies: zero-wait, ideal, hold, regular.
        \begin{enumerate}
            \item Only realistic models, not naive.
            \item Present comparisons between basic strategies, without any additional load: total task duration, time-to-feedback breakdowns, total number of samples.
        \end{enumerate}
        \item Can we do better? Introduce and discuss advanced strategy: adaptive aperiodic approach.
        \begin{enumerate}
            \item Maybe fold in Vishnu's globecom paper here, with modifications to target responsiveness instead of power consumption.
            \item Discuss parameters, and how values were settled on.
            \item Compare adaptive aperiodic with 2 best basic strategies without additional load.
            \item Introduce additional load to showcase the adaptability of the adaptive aperiodic approach.
        \end{enumerate}
    \end{enumerate}
    \item Conclusion
    \begin{enumerate}
        \item Future work and open questions
        \item Effects of individual differences (neuroticism, age, etc)
        \item Extend to other WCAs
        \item Extend to other applications
    \end{enumerate}
\end{enumerate}
\newpage

==> sampling.tex <==
\section{Aperiodic Sampling}

In this section we will explain the method that we used to find the optimum set of sampling instants (or equivalently sampling intervals) for the given distribution of TTE, denoted by $\mathcal{T}$.
\todo[inline]{aka execution times. Need to recheck the terminologies used in this section and make it consistent with the paper.}
We take the modeling and partial solution approach from the recent works on energy efficient sampling of edge-based feedback systems.
In \textcite{ICCperiodic1,TMCperiodic}, the authors model the energy in terms of the expected number of samples $\mathbb{E}[\mathcal{S}]$ and the expected wait time $\mathbb{E}[\mathcal{W}]$ experienced by the user, where the wait time $\mathcal{W}$ --- in the terminology of the authors --- is the time between the event completion and the immediate next sample taken.
The authors then find the optimum periodic sampling interval that minimizes this energy, or equivalently the non-constant parts of this energy termed as \textit{Energy Penalty} $\mathcal{E}$.
In this optimization, the constant parts are excluded as they do not affect the optimization.
With a value much smaller than the execution time of the event or TTE, the RTT of the final sample is included in this constant part, which is the reason why $\mathcal{W}$ is computed without including this RTT.
Next, in \textcite{secAperiodic}, the authors use this exact model and find the optimum aperiodic sampling instants $\{t_n,\,n=1,2,\dots\}$ that minimizes the same energy penalty.
In this work, we use the modeling from \textcite{secAperiodic} to find the optimum aperiodic sampling interval.
However, instead of using their two-step approach to find the solution which include a recursive solution followed by an algorithm, we develop a novel approximate but easier solution to finding the set of optimum aperiodic sampling intervals.
In what follows, we first recap the system modeling used by the authors in \textcite{secAperiodic} and then give our independent approximate solution. 

The energy penalty can be expressed as~\cite{secAperiodic}
\begin{alignat}{1}
\Rightarrow\mathcal{E}&=\alpha\mathbb{E}[\mathcal{S}]+\beta\mathbb{E}[\mathcal{W}],\;\label{eq:epsilon_terminal}
\end{alignat}
where $\alpha\!=\!\tau_{\text{c}} (P_{\text{c}}\!-\!P_0)$ and $\beta\!=\!P_0$ are constants.
\todo[inline]{Define and explain the parameters if this is not done earlier in other sections.}
Here, note that $\alpha\mathbb{E}[\mathcal{S}]$ and $\beta\,\mathbb{E}[\mathcal{W}]$ corresponds to the energy wasted per discarded sample and the additional energy expended for waiting, respectively.
As noted down by the authors, it is important to note that this optimization approach can also be applied to optimize metrics other than energy, simply by formulating this new metrics in the same format as follows, that is by expressing the metric as a linear combination of the expected number of samples $\mathbb{E}[\mathcal{S}]$ and expected wait time $\mathbb{E}[\mathcal{W}]$.
Using this model, we find the approximate, near-optimal set of sampling instants $\{t_n^*\}$ that minimizes the energy penalty given in \cref{eq:epsilon_terminal}.


\subsection{Optimum sampling instants}\label{sec:aprxSol}

First, we borrow the idea of checkpointing density from \textcite{CP_C} and call it instantaneous sampling rate function $r(t)$ which is
related to $\{t_n\}$ such that,
\begin{alignat}{1}
{\int_{t_{n-1}}^{t_n}}r(t)\dif t=1,\;\forall n\geq1.\label{rt}
\end{alignat}
We find $r^*(t)$, the $r(t)$ that minimizes $\mathcal{E}$.
Note that, by construction, the number of samples taken up to any time instant can be computed directly by finding the area under $r(t)$.
Thus, we get the expected number of samples $\mathbb{E}[\mathcal{S}]$ as
\begin{alignat}{1}
\mathbb{E}[\mathcal{S}]&=\int_{t=0}^{\infty}\bigg(\!\int_{x=0}^{t}\!\!\!\!r(x)\,\mathrm{d}x\bigg)f_{\mathcal{T}}(t)\,\mathrm{d}t.\label{Es}
\end{alignat}
To find 
% the expected wait 
$\mathbb{E}[\mathcal{W}]$, we use the TTE conditional CDF.
We get,
\begin{multline*}
\mathbb{P}(\mathcal{W}=t_n-\mathcal{T}\leq t\,\big\vert\,t_{n-1}<\mathcal{T}\leq t_n)\\=\dfrac{\mathbb{P}(\mathcal{T}\geq t_n-t\,,\,t_{n-1}<\mathcal{T}\leq t_n)}{\mathbb{P}(t_{n-1}<\mathcal{T}\leq t_n)}.
\end{multline*}
The numerator is degenerate when $t\!<\!0$ or $t\!>\!(t_n\!-\!t_{n-1})$.
Thus, we are only interested in $0\!\leq\!t\!\leq\! (t_n-t_{n-1})$.
Let $F_{\mathcal{T}}$, $\bar{F}_{\mathcal{T}}$ and $f_{\mathcal{T}}$ corresponds to the CDF, CCDF and pdf of the TTE distribution.
\begin{alignat*}{1}
\!\!\!\Rightarrow\mathbb{P}(\mathcal{W}\leq t\,\big\vert\,t_{n-1}<\mathcal{T}\leq t_n)&=\dfrac{\mathbb{P}(t_n-t\leq\mathcal{T}\leq t_n)}{F_\mathcal{T}(t_n)-F_\mathcal{T}(t_{n-1})}\\
&\approx\dfrac{F_\mathcal{T}(t_n)-F_\mathcal{T}(t_{n}-t)}{F_\mathcal{T}(t_n)-F_\mathcal{T}(t_{n-1})}\tag{$A_1$}\label{Apx1}
\end{alignat*}
Here, \ref{Apx1} is an approximation merely for mathematical maturity due to the slackness of the first inequality in the numerator.
Expanding the CDF using Taylor series, 
\begin{multline*}
    =\Big(F_\mathcal{T}(t_n)-\big(F_\mathcal{T}(t_n)+f_\mathcal{T}(t_n)(-t)+f'_\mathcal{T}(t_n)(-t)^2/2!+\dots\big)\Big)\\
    \div \Big(F_\mathcal{T}(t_n)-\big(F_\mathcal{T}(t_n)+f_\mathcal{T}(t_n)(t_{n-1}-t_n)\\+f'_\mathcal{T}(t_n)(t_{n-1}-t_n)^2/2!+\dots\big)\Big).
\end{multline*}
Simplifying and using the first order approximation, we get
\begin{alignat*}{1}
% &=\dfrac{F_\mathcal{T}(t_n)-\big(F_\mathcal{T}(t_n)+f_\mathcal{T}(t_n)(-t)+f'_\mathcal{T}(t_n)(-t)^2/2!+\dots\big)}{F_\mathcal{T}(t_n)-\big(F_\mathcal{T}(t_n)+f_\mathcal{T}(t_n)(t_{n-1}-t_n)+f'_\mathcal{T}(t_n)(t_{n-1}-t_n)^2/2!+\dots\big)}\\&
\mathbb{P}(\mathcal{W}\leq t\,\big\vert\,t_{n-1}<\mathcal{T}\leq t_n)&\approx\dfrac{tf_\mathcal{T}(t_n)}{(t_{n}-t_{n-1})f_\mathcal{T}(t_n)}\tag{$A_2$}\label{Apx2}\\
\Rightarrow\mathbb{P}(\mathcal{W}> t\,|\,t_{n-1}<\mathcal{T}\leq t_n)&= 1-\dfrac{t}{(t_{n}-t_{n-1})}.
\end{alignat*}
Using this CCDF, we find the conditional expectation of $\mathcal{W}$.
\begin{alignat*}{1}
% \mathbb{P}(\mathcal{W}> t\,|\,t_{n-1}<\mathcal{T}\leq t_n)&\approx 1-\dfrac{t}{(t_{n}-t_{n-1})}\\
\Rightarrow \mathbb{E}[\mathcal{W}\,|\,t_{n-1}<\mathcal{T}\leq t_n]&=\smashoperator[r]{\int_{0}^{t_n-t_{n-1}}}\Big(1-\dfrac{t}{(t_{n}-t_{n-1})}\Big)\,\mathrm{d}t\\
&=\dfrac{(t_n-t_{n-1})}{2}.
\end{alignat*}
% However, we can also approximate $(t_n-t_{n-1})$, the sampling interval to the inverse of the instantaneous sampling frequency $r(t)$. This approximation (\ref{Apx3}) is valid as long as $r(t)$ is varying slowly between two consecutive sampling instants. That is,
If $r(t)$ is varying slowly between two consecutive sampling instants, we can approximate the sampling interval $t_n\!-\!t_{n-1}$ as,
\begin{alignat}{1}
 (t_n-t_{n-1})&\approx\dfrac{1}{r(t)},\;\forall t,n:t_{n-1}\!<\!t\!\leq\!t_n.\tag{$A_3$}\label{Apx3}\\
% \end{alignat}
% As a result, we can compute the expected wait as,
% \begin{alignat}{1}
\Rightarrow \mathbb{E}[\mathcal{W}]&=\int_{0}^{\infty}\mathbb{E}[\mathcal{W}\,|\,t_{n-1}<\mathcal{T}\leq t_n]f_\mathcal{T}(t)\,\mathrm{d}t\nonumber\\
&=\int_{0}^{\infty}\dfrac{1}{2r(t)}f_\mathcal{T}(t)\,\mathrm{d}t.\label{Ew}
\end{alignat}
We can thus find the energy penalty using \eqref{Es} and \eqref{Ew} as
\begin{alignat*}{1}
\mathcal{E}&=\int_{0}^{\infty}\Big(\alpha\int_{x=0}^{t}r(x)\,\mathrm{d}x+\beta\dfrac{1}{2r(t)}\Big)f_{\mathcal{T}}(t)\,\mathrm{d}t.\label{epsilon_eulerForm}\\
\intertext{Let $g(t)=\int_{0}^{t}r(x)\dif x$. Then  $g'(t)=\tfrac{\mathrm{d}}{\mathrm{d}t}g(t)=r(t)$. That is,}
\vspace{-4cm}\mathcal{E}&=\int_{0}^{\infty}\Big(\alpha g(t)+\dfrac{\beta}{2g'(t)}\Big)f_{\mathcal{T}}(t)\,\mathrm{d}t.
\end{alignat*}
As per the Euler-Lagrange equation from the calculus of variations\cite{calcVariation2,calcVariation1}, the extreme value of $\mathcal{E}$ is obtained at 
\begin{alignat}{1}
r^*(t)&=\sqrt{\dfrac{\beta f_\mathcal{T}(t)}{2\alpha\bar{F}_\mathcal{T}(t)}}.\\
\intertext{Thus, for a Rayleigh distributed $\mathcal{T}$ with parameter $\sigma$,}
r^*(t)&=\sqrt{\dfrac{\beta t}{2\alpha\sigma^2}}\\
\Rightarrow &\int_{t_n}^{t_{n+1}}\!\!\!\sqrt{\dfrac{\beta t}{2\alpha\sigma^2}}\,\mathrm{d}t=1,\;\forall n\geq1\nonumber\tag{from \eqref{rt}}\\
\Rightarrow &\;t_{n+1}^{\frac{3}{2}}-t_{n}^{\frac{3}{2}}=3\sigma\!\sqrt{\tfrac{\alpha}{2\beta}}\nonumber\\
\Rightarrow &\;t_n=\Big(3\sigma\!\sqrt{\tfrac{\alpha}{2\beta}}\Big)^{\frac{2}{3}}n^{\frac{2}{3}}.\label{tnFinal}
\end{alignat}

Now, if we have a constrained optimization with an upper bound $w_0$ for the expected wait time, we can find the optimum set of sampling instants by equating \cref{Ew} to $w_0$ and find the ratio of $\frac{\alpha}{\beta}$ that provides the optimum set of sampling instants when plugged into \cref{tnFinal}.
For this, we make use of the facts that
\begin{enumerate*}[itemjoin={{, }}, itemjoin*={{, and }}]
    \item the bound will be tight at the optimum due to the continuous nature of possible sampling instants and sampling intervals
    \item one can achieve any arbitrary point $(\mathbb{E}[\mathcal{S}],\mathbb{E}[\mathcal{W}])$ via the unconstrained optimization discussed above simply by varying the ratio $\frac{\alpha}{\beta}$.
\end{enumerate*}
\begin{alignat*}{1}
\mathbb{E}[\mathcal{W}]&=\int_{0}^{\infty}\dfrac{1}{2r(t)}f_\mathcal{T}(t)\,\mathrm{d}t.\nonumber\\
&=\int_{0}^{\infty}\frac{1}{2}\sqrt{\frac{2\alpha\sigma^2}{\beta t}}\cdot \frac{t}{\sigma^2}e^{-{t^2}/{2\sigma^2}}\mathrm{d}t\\
&=\sqrt{\frac{\alpha\sigma^2}{2\beta}}\int_{0}^{\infty}\frac{\sqrt{t}}{\sigma^2}e^{-{t^2}/{2\sigma^2}}\mathrm{d}t\\
&=\sqrt{\frac{\alpha\sigma^2}{2\beta}}\left({\frac{1}{{2}\sigma^2}}\right)^{1/4}\cdot\int_{0}^{\infty}y^{-1/4}e^{-y}\mathrm{d}y\\
&=\sqrt{\frac{\alpha\sigma^2}{2\beta}}\left({\frac{1}{{2}\sigma^2}}\right)^{1/4}\cdot\mathlarger{\Gamma}(\tfrac{3}{4})\\
% &\approx 0.728637\sqrt{\frac{\alpha\sigma}{\beta}}\\
\intertext{Thus, when the upper bound $w_0$ is tight,}
w_0&=0.728637\sqrt{\frac{\alpha\sigma}{\beta}}\\
w_0&=\sqrt{\frac{\alpha\sigma}{2\sqrt{2}\beta}}\mathlarger{\Gamma}(\tfrac{3}{4})\\
\Rightarrow\frac{\alpha}{\beta}&=\frac{w_0^2}{\sigma}\frac{2\sqrt{2}}{(\mathlarger{\Gamma}(\tfrac{3}{4}))^2}\\&=1.88355\frac{w_0^2}{\sigma}
\end{alignat*}

By making use of this general solution, we can also prove the results given in section \ref{sec:aprxSol_Energy_samples}, where we modify the problem and find the optimum sampling instants that minimises the expected number of samples for a given upper bound $w_0$ for the expected wait time. 
First note that, the general solution has constants $\alpha$ and $\beta$ that corresponds to the weights given to the cost of sampling and cost of waiting, respectively. The optimisation criteria changes from minimising wait time to minimising the number of samples, when the ratio $\frac{\alpha}{\beta}$ goes from zero to infinity. Since any positive real value is valid for this ratio, and since the sampling instants are aperiodic and can take any positive real values, we have
\begin{enumerate*}
    \item the bound will be tight at the optimum due to the continuous nature of possible sampling instants and sampling intervals
    \item one can achieve any arbitrary point $(\mathbb{E}[\mathcal{S}],\mathbb{E}[\mathcal{W}])$ via the unconstrained optimization discussed above simply by varying the ratio $\frac{\alpha}{\beta}$.
\end{enumerate*}
Thus, can argue that any optimisation problem -- constrained or unconstrained -- can be boiled down to modifying the problem to the general format and finding the appropriate $\frac{\alpha}{\beta}$ ratio. Hence, to solve for the modified optimisation problem explained in section \ref{sec:aprxSol_Energy_samples} that minimises $(\mathbb{E}[\mathcal{S}]$ with an upper bound $w_0$ on $(\mathbb{E}[\mathcal{W}]$, we equate \cref{Ew} to $w_0$, find the corresponding $\frac{\alpha}{\beta}$ and find the optimum set of sampling instants by plugging this ratio into \cref{tnFinal}. 

\begin{alignat*}{1}
\mathbb{E}[\mathcal{W}]&=\int_{0}^{\infty}\dfrac{1}{2r(t)}f_\mathcal{T}(t)\,\mathrm{d}t.\nonumber\\
&=\int_{0}^{\infty}\frac{1}{2}\sqrt{\frac{2\alpha\sigma^2}{\beta t}}\cdot \frac{t}{\sigma^2}e^{-{t^2}/{2\sigma^2}}\mathrm{d}t\\
&=\sqrt{\frac{\alpha\sigma^2}{2\beta}}\int_{0}^{\infty}\frac{\sqrt{t}}{\sigma^2}e^{-{t^2}/{2\sigma^2}}\mathrm{d}t\\
&=\sqrt{\frac{\alpha\sigma^2}{2\beta}}\left({\frac{1}{{2}\sigma^2}}\right)^{1/4}\cdot\int_{0}^{\infty}y^{-1/4}e^{-y}\mathrm{d}y\\
&=\sqrt{\frac{\alpha\sigma^2}{2\beta}}\left({\frac{1}{{2}\sigma^2}}\right)^{1/4}\cdot\mathlarger{\Gamma}(\tfrac{3}{4})\\
% &\approx 0.728637\sqrt{\frac{\alpha\sigma}{\beta}}\\
\intertext{Thus, when the upper bound $w_0$ is tight,}
w_0&=0.728637\sqrt{\frac{\alpha\sigma}{\beta}}\\
w_0&=\sqrt{\frac{\alpha\sigma}{2\sqrt{2}\beta}}\mathlarger{\Gamma}(\tfrac{3}{4})\\
\Rightarrow\frac{\alpha}{\beta}&=\frac{w_0^2}{\sigma}\frac{2\sqrt{2}}{(\mathlarger{\Gamma}(\tfrac{3}{4}))^2}\\&=1.88355\frac{w_0^2}{\sigma}
\end{alignat*}


==> tables/empirical_exec_times.tex <==
\begin{table}
\centering
\caption{Random sample of rows from the empirical step execution time data obtained for~\cite{olguinmunoz:impact2021}.}\label{tab:exec_times:empirical}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{rrrrr}
\toprule
subject ID &  step &  exec.\ time &  delay &  neuroticism (norm.) \\
\midrule
\num{136519}      &          \num{116} &               \SI{7.067}{\second} &  \SI{1.650}{\second} &        \num{0.188} \\
\num{135199}      &           \num{12} &             \SI{11.598}{\second} &  \SI{3.000}{\second}&        \num{0.438} \\
\num{136894}      &          \num{101} &               \SI{3.544}{\second} &  \SI{2.700}{\second}&        \num{0.844} \\
\num{134623}      &          \num{138} &               \SI{6.205}{\second} &  \SI{2.175}{\second} &        \num{0.750} \\
\num{136894}      &          \num{127} &               \SI{9.821}{\second} &  \SI{1.650}{\second} &        \num{0.844} \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/processed_exec_times.tex <==
\begin{table*}
    \centering
    \caption{}\label{tab:exectime:proc}
\begin{tabular}{rrrllll}
\toprule
subject ID &  step &  next exec. time & neuroticism &  impairment & transition tag & duration \\
\midrule
\num{136516} &   \num{67} & \SI{4.663}{\second} & medium & high & no transition & short \\
%
\num{137299} &  \num{114} & \SI{2.230}{\second} & low & low & higher-to-lower &  short \\
\num{137344} &   \num{45} & \SI{1.775}{\second} & low &  medium & no transition & medium \\
\num{135955} &   \num{77} & \SI{4.326}{\second} & low &  high & no transition & long \\
\num{135385} &  \num{129} & \SI{2.499}{\second} & high &  medium & no transition & long \\
\bottomrule
\end{tabular}
\todo[inline]{Use same samples as first table for clarity!}
\end{table*}
    
